Modulating the electrochemical intercalation of graphene interfaces with $\alpha$-RuCl$_3$ as a solid-state electron acceptor

Intercalation reactions modify the charge density in van der Waals (vdW) materials through coupled electronic-ionic charge accumulation, and are susceptible to modulation by interlayer hybridization in vdW heterostructures. Here, we demonstrate that charge transfer between graphene and $\alpha$-RuCl$_3$, which dopes the graphene positively, greatly favors the intercalation of lithium ions into graphene-based vdW heterostructures. We systematically tune this effect on Li$^+$ ion intercalation, modulating the intercalation potential, by using varying thicknesses of hexagonal boron nitride (hBN) as spacer layers between graphene and $\alpha$-RuCl$_3$. Confocal Raman spectroscopy and electronic transport measurements are used to monitor electrochemical intercalation and density functional theory computations help quantify charge transfer to both $\alpha$-RuCl$_3$ and graphene upon Li intercalation. This work demonstrates a versatile approach for systematically modulating the electrochemical intercalation behavior of two-dimensional layers akin to electron donating/withdrawing substituent effects used to tune molecular redox potentials.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
